Improved measurements of the Dalitz decays $\eta/\eta'\rightarrow\gamma e^{+}e^{-}$

Based on a data sample of 10 billion $J/\psi$ events collected with the BESIII detector, improved measurements of the Dalitz decays $\eta/\eta'\rightarrow\gamma e^+e^-$ are performed, where the $\eta$ and $\eta'$ are produced through the radiative decays $J/\psi\rightarrow\gamma \eta/\eta'$. The branching fractions of $\eta\rightarrow\gamma e^+e^-$ and $\eta'\rightarrow\gamma e^+e^-$ are measured to be $(7.07 \pm 0.05 \pm 0.23)\times10^{-3}$ and $(4.83\pm0.07\pm0.14)\times10^{-4}$, respectively. Within the single pole model, the parameter of electromagnetic transition form factor for $\eta\rightarrow\gamma e^+e^-$ is determined to be $\Lambda_{\eta}=(0.749 \pm 0.027 \pm 0.007)~ {\rm GeV}/c^{2}$. Within the multi-pole model, we extract the electromagnetic transition form factors for $\eta'\rightarrow\gamma e^+e^-$ to be $\Lambda_{\eta'} = (0.802 \pm 0.007\pm 0.008)~ {\rm GeV}/c^{2}$ and $\gamma_{\eta'} = (0.113\pm0.010\pm0.002)~ {\rm GeV}/c^{2}$. The results are consistent with both theoretical predictions and previous measurements. The characteristic sizes of the interaction regions for the $\eta$ and $\eta'$ are calculated to be $(0.645 \pm 0.023 \pm 0.007 )~ {\rm fm}$ and $(0.596 \pm 0.005 \pm 0.006)~ {\rm fm}$, respectively. In addition, we search for the dark photon in $\eta/\eta^\prime\rightarrow\gamma e^{+}e^{-}$, and the upper limits of the branching fractions as a function of the dark photon are given at 90\% confidence level.

==> acknowledgement_2023-09-11.tex <==
%% Saved at => 2023-09-11
\textbf{Acknowledgement}

The BESIII Collaboration thanks the staff of BEPCII and the IHEP computing center for their strong support. This work is supported in part by National Key R\&D Program of China under Contracts Nos. 2020YFA0406300, 2020YFA0406400; National Natural Science Foundation of China (NSFC) under Contracts Nos. 11635010, 11735014, 11835012, 11935015, 11935016, 11935018, 11961141012, 12025502, 12035009, 12035013, 12061131003, 12192260, 12192261, 12192262, 12192263, 12192264, 12192265, 12221005, 12225509, 12235017; the Chinese Academy of Sciences (CAS) Large-Scale Scientific Facility Program; the CAS Center for Excellence in Particle Physics (CCEPP); Joint Large-Scale Scientific Facility Funds of the NSFC and CAS under Contract No. U1832207; CAS Key Research Program of Frontier Sciences under Contracts Nos. QYZDJ-SSW-SLH003, QYZDJ-SSW-SLH040; 100 Talents Program of CAS; The Institute of Nuclear and Particle Physics (INPAC) and Shanghai Key Laboratory for Particle Physics and Cosmology; European Union's Horizon 2020 research and innovation programme under Marie Sklodowska-Curie grant agreement under Contract No. 894790; German Research Foundation DFG under Contracts Nos. 455635585, Collaborative Research Center CRC 1044, FOR5327, GRK 2149; Istituto Nazionale di Fisica Nucleare, Italy; Ministry of Development of Turkey under Contract No. DPT2006K-120470; National Research Foundation of Korea under Contract No. NRF-2022R1A2C1092335; National Science and Technology fund of Mongolia; National Science Research and Innovation Fund (NSRF) via the Program Management Unit for Human Resources \& Institutional Development, Research and Innovation of Thailand under Contract No. B16F640076; Polish National Science Centre under Contract No. 2019/35/O/ST2/02907; The Swedish Research Council; U. S. Department of Energy under Contract No. DE-FG02-05ER41374

\textbf{Other Fund Information}

To be inserted with an additional sentence into papers that are relevant to the topic of special funding for specific topics. Authors can suggest which to Li Weiguo and/or the physics coordinator.
        Example added sentence: This paper is also supported by the NSFC under Contract Nos. 10805053, 10979059, ....National Natural Science Foundation of China (NSFC), 10805053, PWANational Natural Science Foundation of China (NSFC), 10979059, Lund弦碎裂强子化模型及其通用强子产生器研究National Natural Science Foundation of China (NSFC), 10775075, National Natural Science Foundation of China (NSFC), 10979012, baryonsNational Natural Science Foundation of China (NSFC), 10979038, charmoniumNational Natural Science Foundation of China (NSFC), 10905034, psi(2S)->B BbarNational Natural Science Foundation of China (NSFC), 10975093, D 介子National Natural Science Foundation of China (NSFC), 10979033, psi(2S)->VPNational Natural Science Foundation of China (NSFC), 10979058, hcNational Natural Science Foundation of China (NSFC), 10975143, charmonium rare decays
%% ends here %%

